Robust Large-Margin Learning in Hyperbolic Space

Recently, there has been a surge of interest in representation learning in hyperbolic spaces, driven by their ability to represent hierarchical data with significantly fewer dimensions than standard Euclidean spaces. However, the viability and benefits of hyperbolic spaces for downstream machine learning tasks have received less attention. In this paper, we present, to our knowledge, the first theoretical guarantees for learning a classifier in hyperbolic rather than Euclidean space. Specifically, we consider the problem of learning a large-margin classifier for data possessing a hierarchical structure. We provide an algorithm to efficiently learn a large-margin hyperplane, relying on the careful injection of adversarial examples. Finally, we prove that for hierarchical data that embeds well into hyperbolic space, the low embedding dimension ensures superior guarantees when learning the classifier directly in hyperbolic space.

==> abstract.tex <==
Recently, there has been a surge of interest in representation learning in hyperbolic spaces, driven by their ability to represent hierarchical data with significantly fewer dimensions than standard Euclidean spaces. However, the viability and benefits of hyperbolic spaces for downstream machine learning tasks have received less attention. In this paper, we present, to our knowledge, the first theoretical guarantees for learning a classifier in hyperbolic rather than Euclidean space. Specifically, we consider the problem of learning a \emph{large-margin} classifier for data possessing a hierarchical structure. Our first contribution is a \emph{hyperbolic perceptron} algorithm, which provably converges to a separating hyperplane. We then provide an algorithm to efficiently learn a {large-margin} hyperplane, relying on the careful injection of \emph{adversarial examples}. Finally, we prove that for hierarchical data that embeds well into hyperbolic space, the low embedding dimension ensures superior guarantees when learning the classifier directly in hyperbolic space.


==> body.tex <==
\vspace{-2mm}
\begin{abstract}
\input{abstract.tex}
\end{abstract}

%
\vspace{-2mm}
\section{Introduction}
\label{intro}
\vspace{-1mm}
\input{intro.tex}

% -------------------------------------- %
\vspace{-1mm}
\section{Background and notation}
\vspace{-1mm}
\input{background.tex}

% -------------------------------------- %
%%% Problem setting %%%
\vspace{-1mm}
\section{Hyperbolic linear separator learning}
\vspace{-1mm}
\input{perceptron.tex}

%%% Adversarial learning %%%
\vspace{-1mm}
\section{Hyperbolic large-margin separator learning via adversarial examples}
\label{sec:adv-learning}
\vspace{-1mm}
\input{adversarial.tex}
\vspace{-1mm}
\section{Dimension-distortion trade-off}
\vspace{-1mm}
\label{sec:trade-off}
\input{tradeoff.tex}
\vspace{-2mm}
\section{Experiments}
\label{sec:exp}
\vspace{-1mm}
\input{experiments.tex}
\vspace{-2mm}
\section{Conclusion and future work}
\vspace{-1mm}
\input{conclusion.tex}

%%%%%%%%%%%%%%%%%%%%
\vspace{-3mm}
\section*{Acknowledgements}
\vspace{-2mm}
We thank Pranjal Awasthi for helpful discussions on computing adversarial examples and Eli Chien for helpful comments on an earlier version of the paper.

%%%%%%%%%%%%%%%%%%%%
\vspace{-3mm}
\section*{Broader Impact}
\vspace{-2mm}
The paper proposes novel algorithms for large-margin learning in hyperbolic space. The paper’s scope is theoretical and does not discuss specific applications with societal consequences. Therefore, a discussion of the broader impact of this work is not applicable.


%%%%%%%%%%%%%%%%%%%%%
% Acknowledgements should only appear in the accepted version.
%\section*{Acknowledgements}

% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite
%\nocite{langley00}

\bibliography{ref}
\bibliographystyle{plainnat}

%%%%%%%%%%%%%%%%%%%%%
% Move appendix to separate file
%%%%%%%%%%%%%%%%%%%%%
\newpage
\onecolumn
\appendix

\input{appendix.tex}


==> test.tex <==
\begin{theorem}[Convergence hyperbolic Perceptron in Algorithm~\ref{alg:hyp-svm} (Theorem~\ref{prop:h-perceptron})]
 Assume that there is some $\bar{\vw} \in \R^{d+1}$ with $\sqrt{-\bar{\vw}*\bar{\vw}}=1$ {\color{blue}and $\vw_0 \ast \bar{\vw}  \geq 0$}, and some $\gamma>0$, such that $y_j (\bar{\vw}*\vx_j) \geq \gamma'$ for $j=1, \dots, \vert \mathcal{S} \vert$. Then, Algorithm~\ref{alg:hyp-svm} converges 
in $O\left(\frac{1}{\gamma'}\right)$ steps. {\color{blue}In particular, a margin of $\gamma = \asinh(\gamma')$ is achieved in $O \left( \frac{1}{\sinh(\gamma)}       \right)$.}
\end{theorem}
%
\begin{proof}
Assume wlog $\vw_0 = (0,1, 0, \dots, 0) \in R^{d+1}$. Then $\vw_0 * \vw_0 = -1$, i.e., $\L^d \cap \Hc_{\vw_0} \neq \emptyset$. Hence, $\vw_0$ is a valid initialization. Furthermore, assume that the $t$th error is made at the $j${th} sample, i.e. update $\vv_{t} \gets \vw_t + y_j {\vx}_j$. For $\vu \in \R^{d+1}$, let $\vert \vu \vert = \sqrt{-\vu \ast \vu}$.

Now let us consider two cases:
\begin{itemize}
    \item {\bf Case 1}. In this case, we assume that the normalization is not performed in $t$th step, i.e.,
    $$\vw_{t+1} = \vw_t + y_j {\vx}_j.$$
    Therefore, 
    \begin{align}
    \label{eq:h-perc-case1}
\vw_{t+1} * \bar{\vw} &= (\vw_t + y_j {\vx}_j) * \bar{\vw} =  \vw_t * \bar{\vw} + y_j ({\vx_j}*{\bar{\vw}}) 
\geq \vw_t * \bar{\vw} + {\gamma'}\;.
\end{align}
    \item {\bf Case 2}.~In this case, the normalization is performed in the $t$th step of Algorithm~\ref{alg:hyp-svm}, i.e., $$\vw_{t+1} = \frac{\vw_t + y_j {\vx}_j}{\vert \vw_t + y_j {\vx}_j\vert}$$.
    Thus, 
    \begin{align}
    \label{eq:h-perc-case2}
\vw_{t+1} * \bar{\vw} &= \frac{\vw_t + y_j {\vx}_j}{\vert \vw_t + y_j {\vx}_j\vert} * \bar{\vw} \overset{(i)}{\geq} (\vw_t + y_j {\vx}_j) * \bar{\vw} \geq  \vw_t * \bar{\vw} + \underbrace{y_j ({\vx_j}*{\bar{\vw}}) }_{\geq {\gamma'}}
\geq \vw_t * \bar{\vw} + {\gamma'}\;,
\end{align}
\end{itemize}
where $(i)$ follows as the normalization is performed only if $\vert \vw_t + y_j {\vx}_j\vert < 1$ and numerator is positive by induction.

By utilizing \eqref{eq:h-perc-case1} and \eqref{eq:h-perc-case2}, we obtain the following telescoping sum
\begin{align}
\label{eq:h-perc-step2}
&\quad \sum_{k=0}^{T-1} (-\vw_{k+1}+\vw_k)*\bar{\vw} \leq \sum_{k=0}^{T-1} - {\gamma'} \nonumber \\
&\Rightarrow -\vw_{T} * \bar{\vw} \leq -\vw_0 * \bar{\vw} - T {\gamma'} \; .
\end{align}
Recall that, for the Minkowski product, we have
\begin{align}
\label{eq:h-perc-step1}
\cosh(\measuredangle(\vu,\vu')) &= -\frac{\vu*\vu'}{\sqrt{-\vu*\vu} \; \sqrt{-\vu'*\vu'}} \; =  \frac{-\vu*\vu'}{\vert \vu \vert \; \vert \vu' \vert} \;.
\end{align}

By utilizing \eqref{eq:h-perc-step1} with $(\vu, \vu') = (\vw_{T}, \bar{\vw})$ and $(\vu, \vu') = (\vw_0, \bar{\vw})$ in \eqref{eq:h-perc-step2}, we obtain that 
\begin{align}
\label{eq:h-perc-step3}
\vert \vw_{T} \vert \vert \bar{\vw} \vert \cosh(\measuredangle(\vw_{T},\bar{\vw})) \leq \vert \vw_{0} \vert \vert \bar{\vw} \vert \cosh(\measuredangle(\vw_{0},\bar{\vw})) - T {\gamma'}.
\end{align}
Since, we have $\vert \bar{\vw} \vert = \vert \vw_0 \vert = 1$, it follows from \eqref{eq:h-perc-step3} that 
\begin{align}
\label{eq:h-perc-step4}
\vert \vw_{T} \vert \cosh(\measuredangle(\vw_{T},\bar{\vw})) \leq  \cosh(\measuredangle(\vw_{0},\bar{\vw})) - T {\gamma'}.
\end{align}
Further, using the facts that, due to normalization in Algorithm~\ref{alg:hyp-svm}, $\vert \vw_{T} \vert \geq 1$ and $\cosh(\cdot) \geq 1$, it follows from \eqref{eq:h-perc-step4} that 
\begin{align}
\label{eq:h-perc-step5}
1 \leq  \cosh(\measuredangle(\vw_{0},\bar{\vw})) - T {\gamma'} \overset{(ii)}{\leq} C - T{\gamma'},
\end{align}
where $(ii)$ follows as $\measuredangle (\vw_{i}, \bar{\vw}) < \pi$, since the orientation is fixed by the requirement that $\L^d \cap \Hc_{\vw_i} \neq \emptyset$; as a result, 
we can find an upper bound $\cosh(\measuredangle (\vw_0, \bar{\vw})) < \cosh(\pi) = C$. Now, it follows from \eqref{eq:h-perc-step5} that
\begin{align}
T \leq \frac{C-1}{\gamma'},
\end{align}
\color{blue}
which completes the proof of the convergence guarantee.
The margin is given by
\begin{align*}
    {\rm margin}_{\mathcal{S}}(w)
    = \inf_{(x,y) \in \mathcal{S}} \; \asinh \left( \frac{y(\vw * \vx)}{\sqrt{- \vw * \vw}}  \right) = \asinh(\gamma') \; ,
\end{align*}
which implies that a margin of $\gamma = \asinh(\gamma')$ is achieved in $O \left( \frac{1}{\sinh(\gamma)}  \right)$ steps.
\color{black}
